GO FIGURE: A Meta Evaluation of Factuality in Summarization

While neural language models can generate text with remarkable fluency and coherence, controlling for factual correctness in generation remains an open research question. This major discrepancy between the surface-level fluency and the content-level correctness of neural generation has motivated a new line of research that seeks automatic metrics for evaluating the factuality of machine text. In this paper, we introduce GO FIGURE, a meta-evaluation framework for evaluating factuality evaluation metrics. We propose five necessary and intuitive conditions to evaluate factuality metrics on diagnostic factuality data across three different summarization tasks. Our benchmark analysis on ten factuality metrics reveals that our meta-evaluation framework provides a robust and efficient evaluation that is extensible to multiple types of factual consistency and standard generation metrics, including QA metrics. It also reveals that while QA metrics generally improve over standard metrics that measure factuality across domains, performance is highly dependent on the way in which questions are generated.

==> extended.tex <==
\subsection{Explanations for Conditions of Metric Validity}

We give the full details behind our selection of metric conditions in Table \ref{table:conditions}. 

\begin{table*}[!ht]
 \centering
 \resizebox{.9\linewidth}{!}{%
 \begin{tabularx}{\linewidth}{l*{3}{X}}
 \toprule
 Condition & Definition & Motivation \\ \midrule 
 Boundedness (I) & The metric values should be lower-bounded by completely factually inconsistent summaries and upper-bounded by completely factually consistent summaries. & 
 
 \\ 
Sensitivity (II) & The metric value for a summary should correlate with the level of factuality captured by the summary.  & \\

Robustness (Condition III) & The metric should be \textit{robust} and effective across types of factual errors. & \\

Generality (Condition IV) & The metric should be \textit{generalizable} by satisfying conditions I, II, III and V across domains.  &  \\
Human Correlation (Condition V) & 
The metric should \textit{correlate} with human judgements of factuality. & As noted by prior works on generation evaluation \cite{chaganty-etal-2018-price,Hashimoto2019UnifyingHA}, the scoring function $H(D,S_i)$ represented by human evaluation is a gold standard for assessment of generation quality. It then stands that approximating H is a desirable and \textit{necessary} condition of a factuality metric, however it is not \textit{sufficient} as it does not guarantee distinguishable scores between summaries with similar but varying levels of factual consistency (as enforced by II and I).\\
 \end{tabularx}
 }
 \caption{}
 \label{table:conditions}
\end{table*}
